Lagrangian Cobordism and Fukaya Categories

Given a symplectic manifold M, we consider a category with objects finite ordered families of Lagrangian submanifolds of M (subject to certain additional constraints) and with morphisms Lagrangian cobordisms relating them. We construct a functor that maps this category to a variant of the derived Fukaya category of M in a way that takes into account the triangulated structure of the latter.

==> families-A-infty.tex <==
\subsubsection{Families of $A_{\infty}$-categories and equivalences}
\label{sbsb:families-A-infty}

The discussion here follows Chapter~10 of~\cite{Se:book-fukaya-categ}
where one can find more details and proofs.

Let $\mathcal{A}^i$, $i \in \mathcal{I}$, be a family of
$A_{\infty}$-categories indexed by a set $\mathcal{I}$. Suppose we
also have one $A_{\infty}$-category $\mathcal{A}^{\textnormal{tot}}$
such that for every $i \in \mathcal{I}$, $\mathcal{A}^i$ is a full
$A_{\infty}$-subcategory of $\mathcal{A}^{\textnormal{tot}}$. Denote
the embedding functor by $\mathcal{H}^i : \mathcal{A}^i \to
\mathcal{A}^{\textnormal{tot}}$. We assume further that each
$\mathcal{H}^i$ is a quasi-equivalence. Under these assumption there
exists a family of quasi equivalences $\mathcal{K}^i:
\mathcal{A}^{\textnormal{tot}} \to \mathcal{A}^i$, with $\mathcal{K}^i
\circ \mathcal{H}^i = \textnormal{Id}_{\mathcal{A}^i}$ for every $i
\in \mathcal{I}$. Moreover, the family $\mathcal{A}^i$, $i \in
\mathcal{I}$, admits a structure of a so called {\em coherent system
of $A_{\infty}$-categories} (see~\cite{Se:book-fukaya-categ} for the
precise definition). In particular we obtain a family of
quasi-equivalences $\mathcal{F}^{i_1, i_0}: \mathcal{A}^{i_0} \to
\mathcal{A}^{i_1}$ for every $i_0, i_1 \in \mathcal{I}$ with
$\mathcal{F}^{i,i} = \textnormal{Id}_{\mathcal{A}^i}$ and such that
$\mathcal{F}^{i_2, i_1} \circ \mathcal{F}^{i_1, i_0} \cong
\mathcal{F}^{i_2, i_0}$, where $\cong$ means that the two functors are
isomorphic via a natural transformation. We call the
$A_{\infty}$-functors $\mathcal{F}^{i_1, i_0}$ comparison functors.

Passing to the derived categories $D(\mathcal{A}^i)$, $i \in
\mathcal{I}$, we obtain a coherent system of (ordinary) categories
with equivalences $F^{i_1, i_0}: D(\mathcal{A}^{i_0}) \to
D(\mathcal{A}^{i_1})$ induced from the $\mathcal{F}^{i_1,
i_0}$'s. Moreover, the homology level functors $H(\mathcal{K}^i):
H(\mathcal{A}^{\textnormal{tot}}) \to H(\mathcal{A}^i)$ induced by the
$\mathcal{K}^i$'s uniquely determine the equivalences $F^{i_1, i_0}$.

Of course, the same applies not only to the derived categories
$D(\mathcal{A}^i)$, $i \in \mathcal{I}$, but also to the homological
categories $H(\mathcal{A}^i)$ (which can be viewed as full
subcategories of $D(\mathcal{A}^i)$). Namely, $H(\mathcal{A}^i)$, $i
\in \mathcal{I}$, becomes a coherent system of categories via the same
comparison functors $F^{i_1, i_0}$.



==> floercyl.tex <==
% !TEX root = lcob-2.tex
Let $\overline{W}$ and $\overline{W'}$ be two uniformly monotone
Lagrangians with cylindrical ends.  We will {\em not} assume for now
that they are cylindrically distinct at $\infty$ - see
Definition~\ref{d:cyl-dist} but we do assume that they both satisfy
condition~\eqref{eq:Hlgy-vanishes} (with $\widetilde{M}$ replacing
$M$).

We intend to define the Floer complex
$CF(\overline{W},\overline{W'};\eta; (H,f); \widetilde{\mathbf{J}})$
with coefficients in $\Z_{2}$. We fist describe the data involved in
the definition.

\noindent {\bf A}. The almost complex structure
$\widetilde{\mathbf{J}}=\{ \widetilde{J}_{t}\}_{t\in [0,1]}$.  For a
compact subset $B \subset \mathbb{R}^2$ denote by
$\widetilde{\mathbf{\mathcal{J}}}_B$ the (families of) almost complex
structures $\{ \widetilde{J_t} \}_{t \in [0,1]}$ on $(\widetilde{M},
\widetilde{\omega}) = (\R^{2}\times M, \omega_{0}\oplus \omega)$ with the
following properties:
\begin{enumerate}
  \item For every $t$, $\widetilde{J_t}$ is an
   $\widetilde{\omega}$-tamed almost complex structure on
   $\widetilde{M}$.
  \item For every $t$, the projection $\pi$ is $(\widetilde{J_t},
   i)$-holomorphic on $(\mathbb{R}^2 \setminus B) \times M$.
\end{enumerate}
If $B = \emptyset$ we simply write $\widetilde{\mathbf{\mathcal{J}}}$.

\noindent {\bf B}. The component $\eta\in
\pi_{0}(\mathcal{P}(\overline{W},\overline{W'})$ is fixed as in
\S\ref{sbsb:lag-hf}.

\noindent {\bf C}. The perturbation $(H,f)$.  To describe these
perturbations we first fix the notation for the ends of $\overline{W}$
(see \S\ref{sub:cob-def}).  Thus for $R_{+}$ and $R_{-}$ sufficiently
big we assume
$$\overline{W}|_{[R_+, \infty) \times \mathbb{R}} = 
\coprod_{i=1}^{k_+} [R_+, \infty) \times \{a^+_i\} \times L^{+}_i$$
for some $a^+_1 < \cdots < a^+_{k_+}$ and
$$\overline{W}|_{(-\infty, R_{-}] \times
  \mathbb{R}} = \coprod_{i=1}^{k_-} (-\infty, R_-] \times \{a^-_i\}
\times L^{-}_i$$ for some $a^{-}_1 < \cdots < a^-_{k_-}$.

The couple $(H,f)$ consists of two Hamiltonians $H: [0,1]\times
\widetilde{M}\to \R$ and $f:\R^{2}\to \R$ with the following
properties:
\begin{enumerate}
  \item $D\pi(X^{H_t})=0$ outside $K \times M$ for some compact subset
   $K \subset \mathbb{C}$. In other words, $H_t((x,y), p) \equiv
   H_t(p)$ for $x+iy \in \mathbb{C} \setminus K$, $p \in M$.
  \item The function $f:\R^{2}\to \R$ satisfies:
   \begin{itemize}
     \item[1.] The support of $f$ is contained in the union of the
      sets $$U_{i}^{+}= [R_{+}+1,\infty)\times
      [a^{+}_{i}-\epsilon^{+}_{i}, a^{+}_{i}+\epsilon^{+}_{i}]$$ and
      $$U_{i}^{-}= (-\infty, R_{-}-1]\times
      [a^{-}_{i}-\epsilon^{-}_{i}, a^{-}_{i}+\epsilon^{-}_{i}]~,~$$ where
      the positive constants $\epsilon^{\pm}_{i}$ are small enough
      (and the numbers $R_{+}$ and $R_{-}$ are big enough) so that
      all the sets $U^{\pm}_{i}$ above are pairwise disjoint.
     \item[2.] The restriction of $f$ to each set
      $V_{i}^{+}=[R_{+}+2,\infty)\times [a^{+}_{i}-\epsilon^{+}_{i}/2,
      a^{+}_{i}+\epsilon^{+}_{i}/2]$ and $V_{i}^{-}=(-\infty, R_{+}-2]
      \times [a^{-}_{i}-\epsilon^{-}_{i}/2,
      a^{-}_{i}+\epsilon^{-}_{i}/2]$ is of the form
      $$f(x,y)=\alpha_{i}^{\pm}x+\beta_{i}^{\pm}$$ with
      $\alpha_{i}^{\pm}\in \R$ sufficiently small so that the 
      Hamiltonian isotopy of $\R^{2}$, $\phi^{f}_{t}$, associated to $f$
      keeps the sets $[R_{+}+2,\infty)\times \{a^{+}_{i}\}$ and
      $(-\infty, R_{-}-2]\times \{a^{-}_{i}\}$ inside the respective
      $V_{i}^{\pm}$ for $0\leq t\leq 1$.
     \item[3.] We assume $R_{+}$ and $R_{-}$ sufficiently big so that
      $\overline{W'}$ is cylindrical on $(-\infty, R_{-}]\times \R$ as
      well as on $[R_{+},\infty)\times \R$ and we assume that
      $\epsilon^{\pm}_{i}$ is sufficiently small so that
      \begin{equation}\label{eq:neigh-disj}
         (U_{i}^{+}\backslash ([R_{+}+1,\infty)
         \times \{a^{+}_{i}\}))\cap \overline{W'}=\emptyset
      \end{equation}
      for all indexes $i$ and similarly 
      \begin{equation}\label{eq:neigh-disj2}
         (U_{i}^{-}\backslash ((-\infty, R_{-}-1]\times 
         \{ a^{-}_{i}\} ))\cap \overline{W'}=\emptyset~.~
      \end{equation}
   \end{itemize}
\end{enumerate}
 Notice that the  Hamiltonian flow
$\phi^{e}_{t}$ associated to $e=f\circ \pi$ has the property that
$\phi^{e}_{t}(\overline{W})$ and $\overline{W'}$ are cylindrically
distinct at infinity for all $t\in (0,1]$ whether or not
$\overline{W}$ and $\overline{W'}$ are cylindrically distinct at
infinity to start with.  

We denote by $\mathcal{H}(\overline{W}, \overline{W'})$ the space of
pairs $(H,f)$ as above that have the property that
$\phi^{e}_{1}(\overline{W})$ and $\overline{W'}$ are cylindrically
distinct.  If $\overline{W}$ and $\overline{W'}$ are not cylindrically
distinct at infinity, then the constants $\alpha^{\pm}_{i}$ associated
to those ends of $\overline{W}$ that coincide with some ends of
$\overline{W'}$ satisfy $\alpha^{\pm}_{i}\not=0$ whenever
$(H,f)\in\mathcal{H}(\overline{W}, \overline{W'})$.  In this case the
space $\mathcal{H}(\overline{W},\overline{W'})$ has more than a single
connected component. Each such component is convex, hence
contractible.  These components only depend on $f$ and not on $H$. We
denote the path component of $\mathcal{H}(\overline{W},\overline{W'})$
associated to a pair $(H,f)$ by $[f]$.

Fix $\eta$ as at point {\emph B} above, $(H,f)\in
\mathcal{H}(\overline{W},\overline{W'})$ generic and a generic
$\widetilde{\mathbf{J}} \in \widetilde{\mathbf{\mathcal{J}}}_B$ for
some compact set $B$. The following compactness result is important.
 
Assume that $u:\Sigma \to \mathbb{C} \times M$ is a either a
$\widetilde{J}$-holomorphic curve when $\Sigma$ is either the disk
$D^{2}$ or the sphere $S^{2}$ or a solution of the more general
equation (\ref{eq:Floer-equation}) in case $u$ is a strip.  In case
$\Sigma$ is the disk we assume that $u$ maps the boundary $\partial
\Sigma$ either to $\phi^{e}_{1}(\overline{W})$ or to $\overline{W'}$,
and if $\Sigma$ is the strip, we assume $u(\R\times\{0\})\subset
\phi^{e}_{1}(\overline{W})$, $u(\R\times\{1\})\subset \overline{W'}$.
Let $B'\subset \R^{2}$ be a compact set so that $B\subset B'$ and
$\pi(\phi^{e}_{1}(\overline{W})\cup \overline{W'})\cap ([R_{-}-2,
R_{+}+2]\times \R)\subset B'$.
\begin{lem}\label{lem:open-mapping} 
Assume that the symplectic area of $u$ is finite. Then either
$\pi \circ u$ is constant or $\pi\circ u(\Sigma)\subset B'$.
\end{lem}
The basic argument for this lemma appeared already in \cite{Chek:cob}.
It is a simple application of the open mapping theorem - see
\cite{Bi-Co:cob1} for more details.

In view of this compactness result
 the (standard) construction of the Floer complex
- recalled in~\S\ref{sbsb:lag-hf} - extends without modification to define
$$CF(\phi^{e}_{1}(\overline{W}), 
\overline{W'};\eta'; H;\widetilde{\mathbf{J}})~.~$$
  
Finally, we put
\begin{equation}\label{eq:Floer-cplx-cyl}
   CF(\overline{W},\overline{W'};\eta; (H,f);\widetilde{\mathbf{J}}):= 
   CF(\phi^{e}_{1}(\overline{W}), 
   \overline{W'};\eta'; H;\widetilde{\mathbf{J}}),
\end{equation} 
where $\eta'$ is the path component that corresponds to $\eta$ under
the isotopy $\phi^{e}_{t}$.
 
 
As in~\S\ref{sbsb:lag-hf} we omit the component $\eta$ in case we take
into account all Hamiltonian chords, belonging to all the connected
components of $\mathcal{P}(\overline{W},\overline{W}')$.  The main
property of this variant of Floer homology is as follows, as discussed
in~\cite{Bi-Co:cob1}.
 
\begin{prop} \label{prop:invariance-Fl} \cite{Bi-Co:cob1} The homology
   of the complex $CF(\overline{W},
   \overline{W'};(H,f);\widetilde{\mathbf{J}})$ is independent of $H$,
   $\widetilde{\mathbf{J}}$ and only depends on the path connected
   component $[f]\in \pi_0( \mathcal{H}(\overline{W}, \overline{W'}))$
   up to canonical isomorphism.  We denote this homology by
   $HF(\overline{W},\overline{W'}; [f])$.
   
   If $\phi = \{\phi_t\}_{t \in [0,1]}$ is a horizontal isotopy with
   respect to $\overline{W}$, then there is an isomorphism
   $HF(\overline{W},\overline{W'}; [f])\to
   HF(\phi_{1}(\overline{W}),\overline{W'};\phi_{1}[f])$ that only
   depends on the homotopy class of the path of Hamiltonian
   diffeomorphisms $\phi_{t}$ (with fixed end-points). A similar
   statement is valid if we act with a horizontal isotopy on
   $\overline{W'}$ and keep $\overline{W}$ fixed.
\end{prop}
 
In case $\overline{W}$ and $\overline{W'}$ are distinct at infinity,
then $\mathcal{H}(\overline{W},\overline{W'})$ is path connected and
we may take $f=0$. In this case we denote the homology simply by
$HF(\overline{W},\overline{W'})$.  Moreover, if $\overline{W}$,
$\overline{W'}$ are distinct at infinity and transverse, then for
generic $\widetilde{\mathbf{J}} \in \widetilde{\mathcal{J}}_{B}$ (with
$B$ sufficiently big) the complex $CF(\overline{W}, \overline{W'};
(0,0); \widetilde{\mathbf{J}})$ is well-defined and we denote it by
$CF(\overline{W},\overline{W'}; \widetilde{\mathbf{J}})$.
 


==> functor-F.tex <==
\subsection{The functor $\mathcal{F}$} In this subsection we notice
that the functor $\widetilde{\mathcal{F}}$ can be viewed as a lift of
a functor $\mathcal{F}$ that we define below (this has also been
indicated in \cite{Bi-Co:cob}).

First, denote by $\mathcal{C}ob^{d}_{0,pre}(M)$ the following
category. Its objects are the Lagranagian submanifolds $L\in
\mathcal{L}_{d}^{\ast}(M)$ and the morphisms relating two such objects
$L$ and $L'$ are the cobordisms $V: L\cobto (L_{1},\ldots, L_{k-1},
L')$.  This is easily seen to be a category (obviously non-monoidal).
This will be called the flat (or pre) Lagrangian cobordism category.
There is a projection functor
$$\mathcal{P}:\mathcal{C}ob^{d}_{0}(M)\to \mathcal{C}^{d}_{0,pre}(M)$$  
defined by $\mathcal{P}(L_{1},\ldots, L_{k})=L_{k}$ and which
associates to a morphism $[V]:(L_{1}, L_{2}, \ldots, L_{r})\cobto
(L'_{1},\ldots, L'_{s})$ the connected component $W$ of the cobordims
$V$ that relates $L_{r}$ to the ends $(L'_{q},\ldots , L'_{s})$ so
that all $L'_{q}\cup L'_{q+1}\cup \ldots \cup L'_{s}\cup L_{r}=
\partial W$. Recall also from \S\ref{subsec:cones} that there is a
projection functor $\mathcal{P}:T^{S}D\fuk^{d}(M)\to D\fuk^{d}(M)$. It
is just an immediate reflection of the definitions that there is a
commutative diagram:

$$
\begin{aligned}
   \xymatrix@+0.3in{ \mathcal{C}ob^{d}_{0}(M)\ar[d]_{\mathcal{P}}
     \ar[r]^{\widetilde{\mathcal{F}}} &
     T^{S}D\fuk^{d}(M) \ar[d]^{\mathcal{P}} \\
     \mathcal{C}ob^{d}_{0,pre}(M)\ar[r]^{\mathcal{F}} & D\fuk^{d}(M)}
\end{aligned}
$$

Consider the group $\mathcal{H}am(M)$ of Hamiltonian difeomorphisms of
$M$. It is easy to associate to it the smooth path-groupoid:
$\mathcal{PH}am(M)$. This can be viewed as a category with objects the
elements of $\mathcal{H}am(M)$ and with morphisms the smooth
Hamiltonian isotopies - we use here Moore paths so that composition is
associative.  Given a Lagrangian $L$ in $M$, of particular interest is
the full sub-category $\Omega_{L}\mathcal{H}am(M)$ whose objects are
those Hamiltonian diffeomorphisms $\phi$ so that $\phi(L)=L$.
 
To each Lagrangian $L\in \mathcal{L}^{\ast}_{d}(M)$ we can associate a
functor:
$$\mathcal{L}(L):\mathcal{PH}am(M)\to \mathcal{C}ob^{d}_{0,pre}(M)$$
defined by $\phi \to \phi(L)$ and to a hamiltonian isotopy $\Phi_{t}$
we associate the Lagrangian suspension of $L$ associated to
$\Phi_{t}$.

It is shown in \cite{Ch-Co:cob-Seidel} that, for any $L\in
\mathcal{L}^{\ast}_{d}(M)$, the compostion $\mathcal{F}\circ
\mathcal{L}(L)$ reduces to the Seidel morphism when it is restricted
to $\Omega_{L}\mathcal{H}am(M)$.
 
{\color{red} \begin{rem} Maybe we should say something about this too:
     \begin{itemize}
       \item[i.]$\widetilde{\mathcal{F}}$ as homotopy functor.
       \item[ii.] Grading and going beyond the monotone case.
     \end{itemize}
  \end{rem}}



==> movingbdry.tex <==
\subsection{Moving boundary conditions}
\label{subsubsec:movingbdry}

As before assume that $L_{0}$ and $L_{1}$ are two transverse
Lagrangians. Fix the component $\eta$ and the almost complex structure
$\mathbf{J}$. We also fix once and for all a path $\gamma_{0}$ in the
component $\eta$. Now let $\varphi = \{\varphi_t\}_{t \in [0,1]}$ be a
Hamiltonian isotopy starting at $\varphi_0 = \Id$. The isotopy
$\varphi$ induces a map $$\varphi_* : \pi_0(\mathcal{P}(L_0, L_1))
\longrightarrow \pi_0(\mathcal{P}(L_0, \varphi_1(L_1)))$$ as follows.
If $\eta \in \pi_0(\mathcal{P}(L_0, L_1))$ is represented by
$\gamma:[0,1] \to M$ then $\varphi_* \eta$ is defined to be the
connected component of the path $t \mapsto \varphi_t(\gamma(t))$ in
$\mathcal{P}(L_0, \varphi_1(L_1))$.

The isotopy $\varphi$ induces a canonical isomorphism
\begin{equation} \label{eq:iso-c-phi}
   c_{\varphi}: HF(L_0, L_1; \eta)
   \longrightarrow HF(L_0, \varphi_1(L_1); \varphi_* \eta)
\end{equation}
which comes from a chain level map defined using moving
boundary conditions (see e.g.~\cite{Oh:HF1}). The isomorphism
$c_{\varphi}$ depends only on the homotopy class (with fixed end
points) of the isotopy $\varphi$.

The definition of the isomorphism $c_{\varphi}$ involves some
subtleties due to our use of the universal Novikov ring $\mathcal{A}$
as base ring: given that the symplectic area of the strips with moving
boundaries can vary inside a one parametric moduli space it follows
that the naive definition of the morphism $c_{\varphi}$ - so that each
strip is counted with a weight given by its symplectic area - does not
provide a chain map.  We explain here in more detail the construction
of the map $c_{\varphi}$.

Let $\varphi = \{ \varphi^{H}_{t}\}$ be a Hamiltonian isomorphism
generated by $H$. Denote $L'_1 = \varphi^H_{1}(L_{1})$ and assume that
$L'_1$ is also transverse to $L$ and that the Floer complexes
$C_{1}=CF(L_{0}, L_{1};\eta; 0; \mathbf{J})$ and $C_{2}=CF(L_{0},
L'_1;\varphi_{\ast}\eta; 0;\mathbf{J})$ are well-defined.

Put $\psi_{t}=(\varphi_{t}^{H})^{-1}$. We define the functional
$\Theta_H: \mathcal{P}_{\varphi_{\ast}\eta}(L_{0},L'_1)\to \R$,
$$\Theta_H(\gamma)=\int_{0}^{1}H(\psi_t(\gamma(t))dt
-\int_{0}^{1}H(\gamma_{0}(t))dt~.~$$

Let $\beta:\R\to [0,1]$ be a smooth function so that $\beta(s)=0$ for
$s\leq 0$, $\beta(s)=1$ for $s\geq 1$ and $\beta$ is strictly
increasing on $(0,1)$. Let $x$ be a generator of $C_{1}$. We write
\begin{equation}\label{eq:moving-brdy-sum}
   \tilde{c}_{\varphi}(x)=\sum_{y} \Bigl(\sum_{u} 
   T^{\omega(v_{u})-\Theta_H(y)}\Bigr)y
\end{equation}
with $y$ going over the generators of $C_{2}$ and $u$ going over all
the elements of a zero dimensional moduli space of solutions to
Floer's homogeneous equation $\overline{\partial}_{\mathbf{J}}u=0$ that
start at $x$ and end at $y$ and verify the boundary conditions
$$u(s,0)\subset L_{0} \ , \ u(s,1)\subset \varphi_{\beta(s)}(L_{1})~.~$$
Here the element $v_{u}:\R\times [0,1]\to M$ is defined by the formula
$v_{u}(s,t)=\psi_{t\beta(s)}u(s,t)$ so that $v_{u}(s,t)$ is a strip
with boundary conditions on $L_{0}$ and $L_{1}$.  It is easy to check
that with this definition $\tilde{c}_{\varphi}$ is a chain map.  Note
that the quantity $|\omega(v_{u}) -\omega(u)|$ is bounded by the
variation of $H$ so that $\tilde{c}_{\varphi}$ is well defined over
$\mathcal{A}$. Further, the map $c_{\varphi}$ induced in homology by
$\tilde{c}_{\varphi}$, depends only on the homotopy class with fixed
end points of $\varphi$. Similar constructions can be used to adapt
the rest of the usual Floer theoretic machinery to this moving
boundary situation. They show in particular that $c_{\varphi}$ induces
an isomorphism in homology.
 
\begin{rem} This argument also applies without modification to cases
   when $M$ is not compact (but e.g. tame), if we have some control
   which insures that all solutions $u$ of finite energy as above have
   their image inside a fixed compact set $K \subset M$.
\end{rem}


==> proof-lemma-3.3.2.tex <==
\begin{proof}
   First note that, due to our assumptions on $h$, the subset
   $[-\tfrac{3}{2}, \tfrac{5}{2}] \times \mathbb{R} \times M$ as well
   as its complement are both invariant under the flow
   $\phi_t^{\bar{h}}$ of $\bar{h}$.

   We now define an auxiliary constant. Let $C'>0$ be large enough
   such that the set $B' = [-\tfrac{3}{2}, \tfrac{5}{2}] \times [-C',
   C']$ satisfies the following conditions for every $t \in [0,1]$:
   \begin{enumerate}
     \item $B' \supset (\phi_t^h)^{-1} \Bigl( \pi(V_i) \cap \bigl(
      [-\tfrac{3}{2}, \tfrac{5}{2}] \times \mathbb{R} \bigr) \Bigr)$.
     \item $B' \supset (\phi_t^h)^{-1}(K_{V_1, \ldots, V_{k+1}})$.
     \item $B' \supset (\phi_t^h)^{-1}(\pi(\gamma(t)))$ for every
      chord $\gamma:[0,1] \to \mathbb{C} \times M$ in
      $\mathcal{P}_{\bar{H}_{V_i,V_{i+1}}}$, $i=1, \ldots, k$, and in
      $\mathcal{P}_{\bar{H}_{V_1,V_{k+1}}}$.
   \end{enumerate}

   \noindent \textbf{Step 1.}  {\sl Let $r \in \mathcal{R}^{k+1}$ and
     $u: S_r \to \mathbb{C} \times M$ a solution of~\eqref{eq:jhol1}.
     Define $v:S_r \to \mathbb{C} \times M$ by the formula:
     \begin{equation} \label{eq:nat-v} u(z) =
        \phi_{a_r(z)}^{\bar{h}}(v(z)),
     \end{equation}
     where $a_r:S_r \to [0,1]$ is the transition function. We claim
     that $\textnormal{image\,}(v) \subset B'$.}

   \noindent \textbf{Proof of the claim in Step 1.} A straightforward
   calculation shows that the Floer equation~\eqref{eq:jhol1} for $u$
   transforms into the following equation for $v$:
   \begin{equation}\label{eq:jhol2}
      Dv + J'(z,v)\circ Dv\circ j = Y' + J'(z,v)\circ Y'\circ j.
   \end{equation}
   Here $Y'\in \Omega^{1}(S_{r}, C^{\infty}(TM))$ and $J'$ are defined
   by:
   \begin{equation} \label{eq:nat-Y'-J'} Y=D
      \phi_{a(z)}^{\bar{h}}(Y')+da_r \otimes X^{\bar{h}}, \quad
      J_z=(\phi_{a_r(z)}^{\bar{h}})_{\ast} J'_z.
   \end{equation}
   The map $v$ satisfies the following moving boundary conditions:
   \begin{equation}\label{eq:mov-bdry} \forall \ z \in C_{i}, \quad 
      v(z)\in (\phi_{a(z)}^{\bar{h}})^{-1}(V_{i}).
   \end{equation}
   The asymptotic conditions for $v$ at the punctures of $S_r$ are as
   follows. For $i=1, \ldots, k$, $v(\epsilon_i(s,t))$ tends as $s \to
   -\infty$ to a time-$1$ chord of the flow $(\phi_t^{\bar{h}})^{-1}
   \circ \phi_t^{\bar{H}_{V_i, V_{i+1}}}$ starting on $V_i$ and ending
   on $(\phi_1^{\bar{h}})^{-1}(V_{i+1})$.  (Here $\epsilon_i(s,t)$ is
   the parametrization of the strip-like end at the $i$'th puncture.)
   Similarly, $v(\epsilon_{k+1}(s,t))$ tends as $s \to \infty$ to a
   chord of $(\phi_t^{\bar{h}})^{-1} \circ \phi_t^{\bar{H}_{V_1,
       V_{k+1}}}$ starting on $V_1$ and ending on
   $(\phi_1^{\bar{h}})^{-1}(V_{k+1})$. Note that there exists
   $\delta>0$ (that depends on the function $h$) such those chords
   that lie outside of $[-\tfrac{3}{2} + \delta,
   \tfrac{5}{2}-\delta]\times \mathbb{R} \times M$ have constant
   projection under $\pi$ to points of the type $(-\tfrac{3}{2}, q)$
   or $(\tfrac{5}{2}, q)$, $q \in \mathbb{Z}$.

   \noindent \textbf{Claim 1.a.} {\sl Put $v' = \pi \circ v: S_r \to
     \mathbb{C}$. The map $v'$ is holomorphic over $\mathbb{C}
     \setminus ([-\tfrac{3}{2} + \delta', \tfrac{5}{2}-\delta'] \times
     [-C', C'])$ for small enough $\delta'>0$.}

   Indeed, let $z\in S_r$ be a point with $v'(z) \notin [-\tfrac{3}{2}
   + \delta', \tfrac{5}{2}-\delta'] \times [-C', C']$.  The vector
   field $Y$ from equation~\eqref{eq:jhol1} is of the form
   $Y=Y_{0}+da_r\otimes X^{\bar{h}}$ with $D\pi (Y_{0})=0$ so that for
   $Y'$ we have $Y_{0}=D \phi^{\bar{h}}_{a(z)}(Y')$.  The Hamiltonian
   vector field $X^{\bar{h}}$ is horizontal with respect to $\C\times
   M$, hence $D\pi(Y')=0$. Further, by property iii$^{\ast}$ and the
   definition of $J'$ from~\eqref{eq:nat-Y'-J'} we have that at the
   point $z$ the projection $\pi$ is $(J',i)$-holomorphic. This proves
   claim 1.a.

   Define now the following subsets (see
   Figure~\ref{f:compactness-1}):
   \begin{equation*}
      \begin{aligned}
         & R = \Bigl( \bigcup_{i=1}^{k+1} \bigcup_{t \in [0,1]}
         (\phi_{t}^{h})^{-1}(\pi(V_i)) \Bigr) \cap (\mathbb{C}
         \setminus
         B'), \quad Q = \mathbb{C} \setminus (R \cup B'), \\
         & \mathcal{I} = \Bigl( \bigl \{ (-\tfrac{3}{2}, q) \mid q \in
         \mathbb{Z} \bigr \} \cup \bigl \{ (\tfrac{5}{2}, q) \mid q
         \in \mathbb{Z} \bigr \} \Bigr) \cap B'.
      \end{aligned}
   \end{equation*}
   It is easy to see that $Q \subset \mathbb{C}$ is open and that
   $\overline{R} \subset R \cup \mathcal{I}$.
   \vspace{0.6in}
   \begin{figure}[htbp]
      \begin{center}
         \epsfig{file=compactness-1.eps, width=0.9 \linewidth}
      \end{center}
      \caption{\label{f:compactness-1} The projection to $\mathbb{C}$
        of $V_i$, $V_j$, $\phi_t^{\bar{h}}(V_j)$ and the regions $R$,
        $Q$.}
   \end{figure}
   
   \smallskip
   \noindent \textbf{Claim 1.b.} {\sl $v'(S_r) \cap Q = \emptyset$.}
   \smallskip
   
   To see this, first note that all connected components of $Q$ are
   unbounded, hence none of them has compact closure. Now assume by
   contradiction that $v'(S_r)$ intersects $Q$. Let $Q_{0}$ be one of
   the connected components of $Q$ that intersects $v'(S_{r})$. Note
   that $v'(\partial S_r) \subset B' \cup R$ hence $v'(\partial S_r)
   \cap Q_0 = \emptyset$.  Note also that all the chords corresponding
   to the ends of $v'$ are disjoint from $Q_0$, hence
   $(\overline{v'(S_r)} \setminus v'(S_r)) \cap Q_0 = \emptyset$.
   Finally, $\overline{v'(S_r)}$ is clearly compact. Thus we can apply
   Proposition~\ref{p:open-map} with $w = v'$, $\Sigma = S_r$, $\Gamma
   = \mathbb{C}$ and $U = Q_0$ and obtain that $\overline{Q}_0$ is
   compact. A contradiction. This concludes the proof of claim 1.b.

   \smallskip Note that the intersection points between $\pi(V_i) \cap
   (\mathbb{C} \setminus \textnormal{Int\,} B')$ and
   $\pi(\phi_t^h(V_j)) \cap (\mathbb{C} \setminus \textnormal{Int\,}
   B')$ are all in $\mathcal{I}$.
   
   \noindent \textbf{Claim 1.c.} {\sl Let $P \in \mathcal{I}$. Then
     for every $z \in \textnormal{Int\,}(S_r)$, $v'(z) \neq P$.}
   \smallskip
   
   Indeed, if there were a point $z$ with $v'(z) = P$, then as $v'$ is
   holomorphic in a neighborhood of $z$ the open mapping would imply
   that there is a neighborhood of $P$ which is contained in the image
   of $v'$. But Any neighborhood of $P$ must intersect $Q$, hence we
   obtain a contradiction to claim 1.b. This concludes the proof of
   claim 1.c.
   
   \smallskip

   We are now ready to prove the main statement of Step 1, i.e.
   $\textnormal{image\,}(v') \subset B'$. By what we have proved so
   far, it is enough to show that $\textnormal{image\,}(v') \cap R =
   \emptyset$ which we now proceed to show. Indeed, suppose by contradiction that
   $\textnormal{image\,}(v') \cap R \neq \emptyset$. As all the
   Hamiltonian chords corresponding to $v$ are inside $B' \times M$ we
   have only two possibilities:

   \begin{enumerate}
     \item $\textnormal{image\,}(v') \subset \mathcal{R} \cup
      \mathcal{I}$ and $\textnormal{image\,}(v')$ is not constant at
      one of the points of $\mathcal{I}$.
     \item There exists $z_0, z_1 \in S_r$ with $v'(z_0) \in R$ and
      $v'(z_1) \in B' \setminus \mathcal{I}$.
   \end{enumerate}

   We begin by ruling out possibility 2. Let $\{z_t\}_{t \in [0,1]}$
   be a path in $S_r$ connecting $z_0$ to $z_1$ and such that $z_t \in
   \textnormal{Int\,}(S_r)$ for every $0<t<1$. As $$\partial B' \cap
   \partial R \subset \mathcal{I}$$ it follows that there exists $0<
   t_0 < 1$ such that $v'(z_{t_0}) \in \mathcal{I}$. However, this
   contradicts claim 1.c. This rules out possibility 2.

   Assume now that possibility 1 occurs. Then
   $\textnormal{image\,}(v')$ is entirely contained inside
   $\overline{R_0}$, where $R_0 \subset R$ is one of the connected
   components. Now $\overline{R_0} = R_0 \cup \{P\}$, where $P \in
   \mathcal{I}$. Without loss of generality assume that $P =
   (-\tfrac{3}{2}, q)$ for some $q \in \mathbb{Z}$ (the case $P =
   (\tfrac{5}{2}, q)$ can be dealt with in an analogous way). Note
   that all the Hamiltonian chords that lie in $\overline{R_0} \times
   M$ project via $\pi$ to the point $P$. In particular, at the exit
   puncture of $S_r$, the map $v'$ tends to $P$, i.e.
   \begin{equation} \label{eq:v'-exit} \lim_{s \to \infty}
      v'(\epsilon_{k+1}(s,t)) = P.
   \end{equation}
   Put $v'' = v' \circ \epsilon_{k+1} : [0, \infty) \times [0,1] \to
   \mathbb{C}$. We have $v''(s, 0) \in (-\infty, \tfrac{3}{2}] \times
   \{q\}$ for every $s \geq 0$. We claim that for every $s \geq 0$ we
   have $\partial_s v'' (s,0) \leq 0$. Indeed, if \pbred{$\partial_s
     v''(s_0, 0)>0$} for some $s_0 \geq 0$ then as $v''$ is
   holomorphic we have $\partial_t v''(s_0, 0) = i \partial_s
   v''(s_0,0) \in i \mathbb{R}_{\geq 0}$. It follows that for $t$
   close enough to $0$, $v''(s_0,t) \in Q$. But this contradicts claim
   1.b. Thus, $\partial_s v''(s,0) \leq 0$ for every $s \geq 0$. On
   the other hand we have $\lim_{s \to \infty} v''(s,0) = P$. It
   follows that $v''(s,0) = P$ for every $s \geq 0$. From this it is
   not hard to see (e.g. by a reflection argument) that $v''$ is the
   constant map at $P$. A contradiction. This rules out possibility 1,
   and concludes the proof of Step 1.

   \smallskip 
   \noindent \textbf{Step 2.} We define $C = C_{V_1, \ldots,
     V_{k+1}}>0$ to be a large enough constant so that the subset $B =
   [-\tfrac{3}{2}, \tfrac{5}{2}] \times [-C, C]$ satisfies $$B \supset
   \bigcup_{\tau \in [0,1]} \phi_{\tau}^h(B'),$$ where $B'$ is the
   subset defined in step 1. {\sl We now claim that for every $r \in
     \mathcal{R}^{k+1}$ and every solution $u:S_r \to \mathbb{C}
     \times M$ of~\eqref{eq:jhol1} we have $\textnormal{image\,}(u)
     \subset B \times M$.}

   Indeed, if $u$ is such a solution and we define $v$
   using~\eqref{eq:nat-v} then by step~1 we have $$v(z) \in B' \times
   M, \; \forall z \in S_r.$$ It follows that $$u(z) =
   \phi_{a_r(z)}^{\bar{h}}(v(z)) \in \phi_{a_r(z)}^h (B') \times M
   \subset B \times M, \; \forall z \in S_r.$$
\end{proof}

